Optimal Symmetric Strategies in Multi-Agent Systems with Decentralized Information

We consider a cooperative multi-agent system consisting of a team of agents with decentralized information. Our focus is on the design of symmetric (i.e. identical) strategies for the agents in order to optimize a finite horizon team objective. We start with a general information structure and then consider some special cases. The constraint of using symmetric strategies introduces new features and complications in the team problem. For example, we show in a simple example that randomized symmetric strategies may outperform deterministic symmetric strategies. We also discuss why some of the known approaches for reducing agents' private information in teams may not work under the constraint of symmetric strategies. We then adopt the common information approach for our problem and modify it to accommodate the use of symmetric strategies. This results in a common information based dynamic program where each step involves minimization over a single function from the space of an agent's private information to the space of probability distributions over actions. We present specialized models where private information can be reduced using simple dynamic program based arguments.

==> Coordinator.tex <==
 In this section, we provide a method for finding an optimal symmetric strategy pair using the common information approach of \cite{nayyar2013decentralized}.
 The main idea of the approach is to formulate an equivalent single-agent POMDP problem; solve the equivalent POMDP using a dynamic program; and then translate the results back to the original problem.


Because of Theorem \ref{PROP:ONE}, we will only consider symmetric strategies of the form given in \eqref{eq:structure1}. 
Following the approach in \cite{nayyar2013decentralized},  we construct an equivalent problem by adopting  the point of view of a fictitious coordinator that observes only the common information among the agents (i.e., the coordinator observes  $C_t$), but not the current local states (i.e., $X^i_t,i=1,2$).
The coordinator chooses a single prescription $\Gamma_t$, where $\Gamma_t$ is a mapping from the state space $\mathcal{X}$ to the space of probability distributions over the action space  $\mathcal{U}$. The interpretation of the prescription is that it is a directive to the agents about how they should use their local state information to make the control decisions. Thus, agent $i$ generates its probability distribution over the control space by evaluating the function $\Gamma_t$ on its current local state: 
\begin{align}
    &\delta{U}^i_t=\Gamma_t(X^i_t).\label{commact1}
    \end{align}   

The coordinator chooses its prescription based on the common information. Thus, 
  \begin{align}
    &\Gamma_t=d_t(C_t),
\end{align}
where $d_t$ is referred to as the {coordinator's decision strategy  at time $t$}. The collection of functions $(d_1,...,d_{T})$ is called the coordinator's strategy.  The coordinator's strategy optimization problem is to find a coordination strategy to minimize the expected total cost given by \eqref{eq:cost2}.
The following lemma shows the equivalence of the coordinator's strategy optimization problem and  the original strategy optimization problem for the agents.

\begin{lemma}\label{lem:equi}
Suppose that $(d^{*}_1,...,d^{*}_{T})$ is an optimal strategy for the coordinator. Then, optimal control strategies for the agents in the original problem can be obtained as follows: for $i=1,2$,
\begin{align}
\bar{g}^{*}_t(X^i_{t},C_t)=\Gamma_t(X^i_t) ~~ \mbox{where~}  \Gamma_t=d^{*}_t(C_t).
\end{align}
\end{lemma}
\begin{proof}
The lemma is a direct consequence of the results in \cite{nayyar2013decentralized}.
\end{proof}

Lemma \ref{lem:equi} implies that the agents' strategy optimization problem can be solved by solving the coordinator's strategy optimization problem. The advantage of the coordinator's problem is that it is a sequential decision-making problem with the coordinator as the only decision-maker. (Note that once the coordinator makes its decisions about which prescription to use, the agents act as mere evaluators and not as independent decision-makers.) 

%\blue{Beliefs: Independence and belief update}

%\textbf{Coordinator's belief state:}
As shown in \cite{nayyar2013decentralized}, the coordinator's problem can be viewed as a POMDP. Therefore, the coordinator's belief state can serve as the sufficient statistic for selecting prescriptions. At time $t$, the coordinator's belief is given as:
\begin{align}\label{coord:prob1}
    &\Pi_t(x^{1},x^2)=\prob(X^1_t=x^{1}, X^2_t =x^2|C_t, \Gamma_{1:(t-1)}),
\end{align}
for all $x^1 \in \mathcal{X}, x^2 \in \mathcal{X}$.
Because of the conditional independence property identified in Lemma \ref{LEM:INDEPEN}, the coordinator's beliefs  can be factorized into beliefs on each agent's state, i.e.,
\begin{equation}
    \Pi_t(x^1,x^2)=\Pi^1_t(x^1) \Pi^2_t(x^2),
\end{equation}
where, for $i=1,2,$ $\Pi^i_t$ is the marginal belief on $X^i_t$ obtained from \eqref{coord:prob1}. 

The coordinator can update its beliefs on the agents' states in a sequential manner as described in the following lemma.
% \blue{In terms of marginals}
\begin{lemma}\label{LEM:UPDATE}
For $i=1,2$, $\Pi^i_1$ is the prior belief  on the initial state  $X^i_1$ and for each $t \geq 1$, 
\begin{equation}
    \Pi^i_{t+1}=\eta^i_t(\Pi^i_{t},U_t,\Gamma_t),
\end{equation}
 where   $\eta_t, t \geq 1$, are fixed functions derived from the system model. 
\end{lemma} 
% \red{CHECK: is it the same $\eta$ for both agents? Won't the two belief for the two agents end up being the same always?}
\begin{proof}
% \begin{lemma}\label{LEM:UPDATE}
% For $i=1,2,$ $\Pi^i_1$ is the prior belief ($P_{X^i_1}$) on the initial state  $X^i_1$  and for each $t \geq 1$, 
% \begin{equation}
%     \Pi^i_{t+1}=\eta^i_t( \Pi^i_{t},\Gamma^i_t,U_t),
% \end{equation}

% where   $\eta^i_t$ are fixed functions derived from the system model. (We will use $\eta_t( \Pi^{1,2}_{t},\Gamma^{1,2}_{t},U_t)$ to denote the pair $\eta^1_t( \Pi^1_{t},\Gamma^1_{t},U_t), \eta^2_t( \Pi^2_{t},\Gamma^2_{t},U_t)$.)
% %\red{Shouldn't these by $\beta^i_t$ and $\eta^i_t$? Is the $\beta_t$ notation in DP consistent with this lemma?}
% \end{lemma}
% \begin{proof}
% See Appendix \ref{proof:Coord}.
See Appendix \ref{proof:Coordd}.
\end{proof}

% Finally, we note that given the coordinator beliefs $Pi^1_t$, $Pi^2_t$ and its prescriptions $Gamma^1_t$, $Gamma^2_t$ at time $t$, the joint probability that $Z^{er}_t=\phi$ and $M_t = m_t$ is given as 

% \begin{align}
% &P(Z^{er}_t=\phi, M_t = m_t|\Pi_t^{1,2},\Gamma_t^{1,2}) = \label{eq:probz11}\\
%   & \begin{cases}
%   \sum\limits_{x^{1,2}}\mathds{1}_{\{\Gamma^1_t(x^{1})=0\}}\mathds{1}_{\{\Gamma^2_t(x^{2})=0\}}\Pi^1_t(x^1)\Pi^2_t(x^2) ~~\text{if } m_t = (0,0)\\
%   \sum\limits_{x^{1,2}}p_e\mathds{1}_{\{\Gamma^1_t(x^{1})=m_t^1\}}\mathds{1}_{\{\Gamma^2_t(x^{2})=m_t^2\}}\Pi^1_t(x^1)\Pi^2_t(x^2) ~~ \text{otherwise}.
%   \end{cases}\notag
% \end{align}
% Similarly, the probability that $Z^{er}_t = (x^1,x^2)$ is given as 

% \begin{align}
%     &P(Z^{er}_t=(x^1,x^2)|\Pi_t^{1,2},\Gamma_t^{1,2})\notag\\
%     &~~=(1-p_e)\Big[\max(\Gamma^1_t(x^{1}),\Gamma^2_t(x^{2}))\Big]\Pi^1_t(x^1)\Pi^2_t(x^2). \label{eq:probz22}
%  \end{align}
 

% \textbf{Coordinator's dynamic program:} Using Lemma 3 and the probabilities given in \eqref{eq:probz11} - \eqref{eq:probz22}, we can write a dynamic program for the coordinator's POMDP problem. In the following theorem, $\pi^i$ denotes a general probability distribution on $\mathcal{X}^i$ and $\delta_{x^i}$ denotes a delta distribution centered at $x^i$.



% \begin{theorem}\label{thm:dp}
% The value functions  for the coordinator's dynamic program are as follows: for all beliefs $\pi^1,\pi^2,$ $V_{T+1}(\pi^1,\pi^2):=0$ and for  $t=T, \ldots, 2, 1,$ 
%  \begin{align}
%   &V_{t^+}(\pi^1,\pi^2) := \notag \\
%  &\min_{\lambda^1, \lambda^2} \Big[\Big(\sum_{x^{1,2}}c_t\big(x^{1,2},\lambda^1(x^{1}),\lambda^2(x^{2})\big)\pi^1(x^1)\pi^2(x^2)\Big) \notag\\
%  &+V_{t+1}(\beta_t( \pi^{1,2},\lambda^{1,2}))\Big],
% \end{align}
% where $\beta_t$ is as described in Lemma \ref{LEM:UPDATE}.
% \begin{align}
%   &V_{t}(\pi^1,\pi^2) := \label{dyn:update}\\
%  &\min_{\gamma^1, \gamma^2}\Big[\sum_{x^{1,2}}\rho(x^{1,2})\max(\gamma^1(x^{1}),\gamma^2(x^{2}))\pi^1(x^1)\pi^2(x^2) \notag \\ 
% &+\sum_{m}P(Z^{er}_t=\phi,M_t = m|\pi^{1,2},\gamma^{1,2}) V_{t^+}(\eta_t( \pi^{1,2},\gamma^{1,2}, \phi,m))\notag \\
% &+\sum_{\tilde{x}^{1,2}}P(Z^{er}_t=\tilde{x}^{1,2}|\pi^{1,2},\gamma^{1,2})V_{t^+}(\delta_{\tilde{x}^1},\delta_{\tilde{x}^2})\Big],\notag
% \end{align}
% % where $\eta_t$ is as described in Lemma \ref{LEM:UPDATE} and $P(Z^{er}_t=\phi,M_t = m|\pi^{1,2},\gamma^{1,2})$, $P(Z^{er}_t=\tilde{x}^{1,2}|\pi^{1,2},\gamma^{1,2})$ are as described in \eqref{eq:probz11} - \eqref{eq:probz22}. The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1,\pi^2)$.
% \end{theorem}
% \begin{proof}
% Since the coordinator's problem is a POMDP, it has a corresponding dynamic program. The value functions in the theorem can be obtained by simple manipulations of the POMDP dynamic program for the coordinator. 

% \end{proof}

% \begin{remark}\label{infiniteremark}
% We can consider an infinite-horizon discounted cost analog of the problem formulation in this paper wherein the transition and cost functions are time-invariant. The results above can be extended to this discounted setting in a straightforward manner using the approach in \cite{nayyar2013decentralized}.
% \end{remark}

\section{Dynamic Programming for full information and reduced information structure}
Using Lemma \ref{LEM:UPDATE} and the results in \cite{nayyar2013decentralized}, we can write a dynamic program for the coordinator's POMDP problem. 
% \red{why is this sentence here? In the following theorem, $\pi^i$ denotes a general probability distribution on $\mathcal{X}$.}


\begin{theorem}\label{thm:dp}
Let $\mathcal{B}$ be the space of functions from $\mathcal{X}$ to $\Delta(\mathcal{U})$. For a $\gamma \in \mathcal{B}$ and $x \in \mathcal{X}$, $\gamma(x)$ is a probability distribution on $\mathcal{U}$. Let $\gamma(x;u)$ denote the probability assigned to $u \in \mathcal{U}$ under the probability distribution $\gamma(x)$.
The value functions  for the coordinator's dynamic program are as follows: for any realization $\pi^1_t,\pi^2_t$ of $\Pi^1_t,\Pi^2_t$ respectively, define
% \begin{align}
%   &V_{T}(\pi^1_T,\pi^2_T) :=\min_{\gamma_T}E[c_T(X_T,U_T)|\Pi^{1,2}_T=\pi^{1,2}_T,\Gamma_T=\gamma_T]
%  \end{align}
%  and for $t=T-1,\cdots,1$,
%  \begin{align}
%     &V_{t}(\pi^1_t,\pi^2_t) :=\notag\\ &\min_{\gamma_t}E[c_t(X_t,U_t)+V_{t+1}(\pi_{t+1})|\Pi^{1,2}_t=\pi^{1,2}_t,\Gamma_t=\gamma_t]
%  \end{align}
 \begin{align}
  V_{T}(\pi^1_T,\pi^2_T) :=\min_{\gamma_T \in \mathcal{B}}\sum_{x^{1,2}}\sum_{u^{1,2}} c_T(x^{1,2},u^{1,2})&\pi^1_T(x^{1})\pi^2_T(x^{2}) \notag\\
  \times \gamma_T(x^{1};u^1)&\gamma_T(x^{2};u^2)
 \end{align}
%  \red{Has the $gamma(\cdot ; \cdot)$ notation been defined?}
 and for $t=T-1,\cdots,1$,
 \begin{align}
    &V_{t}(\pi^1_t,\pi^2_t) :=\min_{\gamma_t \in \mathcal{B}}\sum_{x^{1,2}}\sum_{u^{1,2}}\pi^1_t(x^{1})\pi^2_t(x^{2})\gamma_t(x^{1};u^1)\gamma_t(x^{2};u^2)\notag\\
    &\times[c_t(x^{1,2},u^{1,2})+V_{t+1}(\eta^1_t( \pi^1_{t},\gamma_t,u_t),\eta^2_t( \pi^2_{t},\gamma_t,u_t))]
 \end{align}
%  \red{$V_{t+1}$  should have two arguments like $V_t$}
 The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1_t,\pi^2_t)$.
\end{theorem}
% \red{we should define the space of prescriptions at the beginning of the theorem and change min over gamma to min over $\gamma \in $ that space}
\begin{proof}
Since the coordinator's problem is a POMDP, it has a corresponding dynamic program. The value functions in the theorem can be obtained by simple manipulations of the POMDP dynamic program for the coordinator. 

\end{proof}


\begin{theorem}\label{thm:dp}
Let $\mathcal{\tilde{B}}$ be the space of functions from $\mathcal{X}^{1:t}$ to $\Delta(\mathcal{U})$. For a $\sigma \in \mathcal{\tilde{B}}$ and $x_{1:t} \in \mathcal{X}^{1:t}$, $\sigma(x_{1:t})$ is a probability distribution on $\mathcal{U}$. Let $\sigma(x_{1:t};u)$ denote the probability assigned to $u \in \mathcal{U}$ under the probability distribution $\sigma(x_{1:t})$.
The value functions  for the coordinator's dynamic program are as follows: for any realization $\lambda^1_t,\lambda^2_t$ of $\Lambda^1_t,\Lambda^2_t$ respectively, define
% \begin{align}
%   &V_{T}(\pi^1_T,\pi^2_T) :=\min_{\gamma_T}E[c_T(X_T,U_T)|\Pi^{1,2}_T=\pi^{1,2}_T,\Gamma_T=\gamma_T]
%  \end{align}
%  and for $t=T-1,\cdots,1$,
%  \begin{align}
%     &V_{t}(\pi^1_t,\pi^2_t) :=\notag\\ &\min_{\gamma_t}E[c_t(X_t,U_t)+V_{t+1}(\pi_{t+1})|\Pi^{1,2}_t=\pi^{1,2}_t,\Gamma_t=\gamma_t]
%  \end{align}
 \begin{align}
  V_{T}(\lambda^1_T,\lambda^2_T) :=\min_{\sigma_T \in \mathcal{\tilde{B}}}\sum_{x^{1,2}_{1:T}}\sum_{u^{1,2}_T} c_T(x^{1,2}_T,u^{1,2}_T)&\lambda^1_T(x^{1}_{1:T})\lambda^2_T(x^{2}_{1:T}) \notag\\
  \times \sigma_T(x^{1}_{1:T};u^1_t)&\sigma_T(x^{2}_{1:T};u^2_t)
 \end{align}
%  \red{Has the $gamma(\cdot ; \cdot)$ notation been defined?}
 and for $t=T-1,\cdots,1$,
 \begin{align}
    &V_{t}(\lambda^1_t,\lambda^2_t) :=\notag\\
    &\min_{\sigma_t \in \mathcal{\tilde{B}}}\sum_{x^{1,2}_{1:t}}\sum_{u^{1,2}_t}\lambda^1_t(x^{1}_{1:t})\lambda^2_t(x^{2}_{1:t})\sigma_t(x^{1}_{1:t};u^1_t)\sigma_t(x^{2}_{1:t};u^2_t)\notag\\
    &\times[c_t(x^{1,2}_t,u^{1,2}_t)+V_{t+1}(\beta^1_t( \lambda^1_{t},\sigma_t,u_t),\beta^2_t( \lambda^2_{t},\sigma_t,u_t))]
 \end{align}
%  \red{$V_{t+1}$  should have two arguments like $V_t$}
 The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\lambda^1_t,\lambda^2_t)$.
\end{theorem}
% \red{we should define the space of prescriptions at the beginning of the theorem and change min over gamma to min over $\gamma \in $ that space}
\begin{proof}
Since the coordinator's problem is a POMDP, it has a corresponding dynamic program. The value functions in the theorem can be obtained by simple manipulations of the POMDP dynamic program for the coordinator. 

\end{proof}


\section{Special Cases}
\subsection{IID local states and controlled global state}

% two lemmas clearly describing $\pi$ and $\lambda$ evolution. In particular $\lambda_{t+1}(x^1_{1:t+1})$ is equal to $\alpha(x^1_{t+1})*\omega_{t+1}(x^1_{1:t})$ where $\omega_{t+1}$ is a function of $\Lambda_t,\Sigma_t,Z_{t+1},U_t$

\begin{lemma}\label{LEM:UPDATE}
For $i=1,2$, $\alpha$ is the prior belief  on the initial state  $X^i_1$ and for each $t \geq 1$, 
\begin{equation}
    \Pi^i_{t+1}(x^i_{t+1})=\alpha(x^i_{t+1}),
\end{equation}
\end{lemma}
\begin{lemma}\label{LEM:UPDATE}
For $i=1,2$, $\Lambda^i_1$ is the prior belief  on the initial state  $X^i_1$ and for each $t \geq 1$, 
% \begin{equation}
%     \Lambda^i_{t+1}(x^i_{1:t+1})=\alpha(x^i_{t+1})\times\omega_t(\Lambda^i_t,\Sigma_t,Z_{t+1},U_t),
% % \end{equation}
% \begin{equation}
%     \Lambda^i_{t+1}(x^i_{1:t+1})=\alpha(x^i_{t+1})\times\omega_t(\Lambda^i_t,\Sigma_t),
% \end{equation}
 \begin{align}
    %   \lambda^1_{t+1}(x^1_{1:t+1})=\alpha(x^1_{t+1})\times[\omega_t(\lambda^1_t,\sigma_t,u^1_t)](x^1_{1:t})
    \lambda^1_{t+1}(x^1_{1:t+1})=\alpha(x^1_{t+1})\times\tilde{\lambda}^1_t(x^1_{1:t}).
  \end{align}
  where $\tilde{\lambda}^1_t =\omega_t(\lambda^1_t,\sigma_t,u^1_t)$ is the belief on agent $1's$ state history until time $t$ after observing $u^1_t$ and $\omega$ is defined as follows:
  \begin{align}
      [\omega_t(\lambda^1_t,\sigma_t,u^1_t)](x^1_{1:t})=\frac{\sigma_t(x^1_{1:t};u^1_t)\lambda^1_{t}(x^1_{1:t})}{\sum_{\Tilde{x}^1_{1:t}}\sigma_t(\Tilde{x}^1_{1:t};u^1_t)\lambda^1_{t}(\Tilde{x}^1_{1:t})}
  \end{align}
  
%  where   $\omega_t, t \geq 1$, are fixed functions derived from the system model. 
\end{lemma} 
\begin{proof}
See Appendix \ref{proof2:Coordd}
\end{proof}
Suppose $\gamma^*$ is the optimal prescription in the reduced DP, can we show $Q^f(\lambda,\sigma)\ge Q^f(\lambda,\gamma^*)$ for any arbitrary $\sigma$ 
\subsection{Notes}
Common information includes past local states in addition to earlier CI

\subsection{Special Dynamics}\label{Special Dynamics}
\input{special_dynamics}

\subsection{Special Cost structure}\label{special cost}
\input{special_cost}
% $c(x^1,x^2,u^1,u^2)\ge 0$ \\
% for each $x^i$ there is $m(x^i)$ such that $c(x^1,x^2,m(x^1),m(x^2))=0$



==> Shared_state.tex <==
In our formulation in Section \ref{sec:problem_formulation}, state of each agent had a single component i.e. the local state. In this section, we consider an extension where the state of each agent has two components: a local state and a shared state identical to all agents. The shared state $Z_t \in \mathcal{Z}$, which is identical to all agents. The initial shared state $Z_1$ has a distribution $P_Z$. Conditioned on the initial shared state $Z_1$, the initial local state of all subsystems are independent.

For the model defined in section \ref{Shared state}, system dynamics, information structure, cost function and common information is defined as follows:

System Dynamics: The shared and the local state of each agent are coupled through the control actions; the shared state evolves according to
\begin{equation}\label{eq:shareddyna}
    Z_{t+1}=f^o_t(Z_{t},U_t,W^o_t), 
\end{equation}
The local state of agent $i$, $i=1,2$, evolves according to 
\begin{equation}\label{eq:shareddyna2}
    X^i_{t+1}=f_t(X^{i}_{t},Z_t,U_t,W^i_t), 
\end{equation}
Equation \eqref{eq:shareddyna2} is similar to \eqref{eq:dyna}, but in case of \eqref{eq:shareddyna2} the next local state of each agent depends on its own current local state, current shared state and control actions of both the agents.

Information structure: The information available to agent $i$ at time $t$ is given by 
\begin{equation}\label{eq:newinfostr}
    I^i_{t}=\{X^i_{1:t},Z_{1:t},U_{1:t-1}\}.
\end{equation}


Cost function: At time $t$, the system incurs a cost $k_t(X^1_t,X^2_t,Z_t,U^1_t,U^2_t)$ that depends on the local states, shared state and control actions of both agents.
% In addition, a communication cost $\rho$ is incurred each time the agents share local states with each other.
The system runs for a time horizon $T$. The total expected cost associated with a  strategy pair $(g^1,g^2)$ is given by 
\begin{equation}\label{eq:newcost2}
  J(g^1,g^2):=\ee^{(g^1,g^2)}\left[\sum_{t=1}^{T}k_t({X}_t,Z_t,{U}_t)\right].
\end{equation}
Our goal is to find a symmetric strategy pair that achieves the minimum total expected cost among all symmetric strategy pairs.

Common information: At time  $t$, $C_t$ is defined as 
\begin{align}
C_t:=(U_{1:t-1},Z_{1:t}),\label{eq:newcommoninfo}
\end{align}
Lemma \ref{LEM:INDEPEN} and Theorem \ref{PROP:ONE} applies to the above defined model with few modifications.
\begin{lemma}[Conditional independence property] \label{LEM:INDEPEN1}
Consider any arbitrary (symmetric or asymmetric) choice of agents' strategies. Then, at any time $t$, the two agents'  local states are conditionally independent given the common information $C_t=(Z_{1:t},U_{1:t-1})$. That is, if $c_t=(z_{1:t},u_{1:t-1})$ is the realization of the common information at time $t$ then for any realization ${x}_{1:t}$ of states, we have
\begin{equation}\label{eq:newindepen}
    \prob^{(g^1,g^2)}({x}_{1:t}|z_{1:t},u_{1:t-1})=\displaystyle\prod_{i=1}^{2} \prob^{g^i}(x^{i}_{1:t}|z_{1:t},u_{1:t-1}), 
    \end{equation}
    Further, $\prob^{g^i}(x^{i}_{1:t}|z_{1:t},u_{1:t-1})$ depends only on agent $i$' strategy and not on the strategy of agent $-i$.
\end{lemma}    
\begin{proof}
This lemma is similar to Lemma \ref{LEM:INDEPEN} except that the common information now includes the shared state history.
\end{proof}
The following theorem shows that agents can ignore their past local states  without losing optimality.
\begin{theorem} \label{PROP:TWO}
 Agents can use symmetric strategies of the form below
\begin{equation} \label{eq:newstructure1}
   \delta{U}^i_t= \bar{g}_t(X^i_{t},Z_{1:t},U_{1:t-1}), ~~ i=1,2,
\end{equation}
without loss of optimality.  In other words, at time $t$, agent $i$ does not need its past local states, $X^i_{1:t-1}$, for making optimal decisions.
\end{theorem}
\begin{proof}
This Theorem is similar to Theorem \ref{PROP:ONE} except with few modifications in the proof which includes the shared state history in the common information.
\end{proof}
Our main objective is to find symmetric control strategies for the agents in the above setup. With some minor modifications, we can use the common information based methodology of Section \ref{Coordinator Results} to solve this problem. 
The following theorem describes the modified dynamic program for the coordinator.
\begin{theorem}\label{thm:dp2}
Let $\mathcal{B}$ be the space of functions from $\mathcal{X}$ to $\Delta(\mathcal{U})$. The value functions  for the coordinator's dynamic program are as follows: for any realization $\pi^1_t,\pi^2_t$ of $\Pi^1_t,\Pi^2_t$ respectively, define
% \begin{align}
%   &V_{T}(\pi^1_T,\pi^2_T) :=\min_{\gamma_T}E[c_T(X_T,U_T)|\Pi^{1,2}_T=\pi^{1,2}_T,\Gamma_T=\gamma_T]
%  \end{align}
%  and for $t=T-1,\cdots,1$,
%  \begin{align}
%     &V_{t}(\pi^1_t,\pi^2_t) :=\notag\\ &\min_{\gamma_t}E[c_t(X_t,U_t)+V_{t+1}(\pi_{t+1})|\Pi^{1,2}_t=\pi^{1,2}_t,\Gamma_t=\gamma_t]
%  \end{align}
 \begin{align}
  V_{T}(\pi^1_T,\pi^2_T) :=\min_{\gamma_T \in \mathcal{B}}\sum_{x^{1,2}}\sum_{z}\sum_{u^{1,2}} c_T(x^{1,2},z,u^{1,2})&\times \notag\\
  \times \pi^1_T(x^{1})\pi^2_T(x^{2})\gamma_T(x^{1};u^1)&\gamma_T(x^{2};u^2)
 \end{align}
%  \red{Has the $gamma(\cdot ; \cdot)$ notation been defined?}
 and for $t=T-1,\cdots,1$,
  \begin{align}
  &V_{t}(\pi^1_t,\pi^2_t) :=\notag\\
    &\min_{\gamma_t \in \mathcal{B}}\sum_{x^{1,2}}\sum_{z}\sum_{u^{1,2}}\pi^1_t(x^{1})\pi^2_t(x^{2})\gamma_t(x^{1};u^1)\gamma_t(x^{2};u^2)\notag\\
    &\times[c_t(x^{1,2},z,u^{1,2})+V_{t+1}(\eta^1_t( \pi^1_{t},\gamma_t,u_t),\eta^2_t( \pi^2_{t},\gamma_t,u_t))]
 \end{align}
 The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1_t,\pi^2_t)$.
\end{theorem}



==> introduction.tex <==
% \blue{List of points required for intro:}

% \begin{itemize}
%   \item  \blue{The problem of sequential decision-making by a team of collaborative agents has received significant attention in the recent literature.}
%  \item \blue{Motivation for symmetric strategies: Simplicity, identity unknown in a varying population setup.}  
%   \item  \blue{Control sharing information structures arise naturally in many
% communication applications such as multi-access broadcast \cite{ooi1996decentralized} and real-time
% communication with feedback \cite{walrand1983optimal}.}
% \item \blue{Control sharing information structure is a special case of partial history sharing information structure.}

% \item \blue{Randomized actions in case of team problems.}

% \end{itemize}

The problem of sequential decision-making by a team of collaborative agents has received significant attention in the recent literature\cite{szer2012maa,seuken2008formal,kumar2015probabilistic,dibangoye2016optimally,rashid2018qmix,hu2019simplified}. The goal in such problems is to jointly design decision/control strategies for the multiple agents in order to optimize a performance metric for the team \cite{nayyar2010optimal, nayyar2013decentralized, mahajan2013optimal,sudhakara2021optimal}.

In multi-agent problems, in many cases we essentially have identical agents, identical action spaces and local state spaces. In this paper, we investigate the problem of designing symmetric control strategies for multiple agents in the team. There are two major motivations for using symmetric strategies and one of them is simplicity. Instead of designing $n$ different strategies for $n$ agents we need to design just one strategy for all agents in the team. The other main motivation for the agents to use symmetric strategies is when they don't have any individualized identities, i.e. in a setting where the population of the agent is not fixed and agents are unaware of their indices \cite{neely2021repeated}.The agents in our current problem formulation are not labeled, so the first agent cannot distinguish itself as "agent 1" and the second cannot distinguish itself as "agent 2". In this kind of problem it makes sense to have a symmetric decision making strategy that applies for all agents, irrespective of their index. Since the agents in the team are restricted to use symmetric strategies, it would be helpful to use randomized actions in our problem.

Control sharing is one kind of information structure which we use in our paper to address the problem \cite{ooi1996decentralized,walrand1983optimal}. Control sharing information structure is a special case of partial history sharing information structure. Our model is similar to the fully observed model in \cite{mahajan2013optimal}.
% Control sharing information structures arise naturally in many
% communication applications such as multi-access broadcast \cite{ooi1996decentralized} and real-time
% communication with feedback \cite{walrand1983optimal}. 
% \blue{Our model is similar to the fully observed model in \cite{mahajan2013optimal}, except the shared state $Z_t$ which is identical for all agents. In our model the shared state $Z_t=\varnothing$.}
The model considered in \cite{mahajan2013optimal} is a discrete-time networked control system with $n$ agents. The state of each agent has two components: a local state and a shared state identical to all agents. The shared and the local state of each agent are coupled through the control actions. The next shared state depends on the current shared state and the control actions of both the agents. While the next local state of each agent depends on its own current local state, current shared state and control actions of both the agents.

\blue{\textit{Organization:}The rest of the paper is organized as follows. We formulate the team problem in Section \ref{sec:problem_formulation} and explain in detail the private information reduction in Section \ref{Preliminary_Results}. In Section \ref{Coordinator Results}, we provide a method for finding an optimal symmetric strategy pair using the common information approach. In Section \ref{Shared state}, we analyze the model with shared state and provide a dynamic programming characterization of the value. We conclude the paper in Section \ref{sec:conclusion}. Proofs of key results are provided in the appendices.}

\blue{In italics Contributions: Main contributions-private info. reduction
}
% Our model is similar to the fully observed model in \cite{mahajan2013optimal}, but unlike \cite{mahajan2013optimal} we do not have an additional shared state identical to all the agents. 



==> prelim_results.tex <==
In this section, we show that there is an optimal symmetric strategy pair that ignores a lot of information available to the agents. To do so, we first split the information available to the agents into two parts -- common information (which is available to both agents) and private information (which is available to only one agent). 
At time  $t$, the common information is defined as 
\begin{align}
C_t:=U_{1:t-1},\label{commoninfo}
\end{align}
and the private information for agent $i$, $i=1,2,$ is defined as 
\begin{align}
P_t^i &:= I_t^i \setminus C_t  = X^i_{1:t}.
\end{align}

Our goal is to reduce agents' private information without compromising the performance achievable under symmetric strategies. One approach for reducing private information that has been commonly used in prior literature on multi-agent/decentralized systems is called the agent-by-agent (or person-by-person approach). 
This approach works as follows: We start by fixing agent $-i$'s strategy to an arbitrary choice and then show that agent $i$ can make decisions based on a subset or a function of its private information without compromising performance. If this reduction in agent $i$'s information holds for any arbitrary strategy of agent $-i$, we can conclude that this reduction would hold for globally optimal strategy as well.  The problem with this approach, however, is that it cannot accommodate the restriction to symmetric strategies. The approach allows agents to use different strategies and the only conclusion it can make is that agents can use strategies with reduced information but these reduced-information strategies may or may not be symmetric. Thus, we cannot adopt this approach for reducing agents' private information in our problem. \red{counter-example}


We will adopt a constructive approach for reducing private information for symmetric strategies in our setup. For \emph{any given pair of symmetric strategies}, we will construct another pair of symmetric strategies with the \emph{same performance and reduced private information}. It then follows that agents can be restricted to use  symmetric strategies with reduced private information without compromising performance.

To proceed, we will need   a key conditional independence property established in the following lemma.

\begin{lemma}[Conditional independence property] \label{LEM:INDEPEN}
Consider any arbitrary (symmetric or asymmetric) choice of agents' strategies. Then, at any time $t$, the two agents'  local states are conditionally independent given the common information $C_t$. That is, if $c_t$ is the realization of the common information at time $t$ then for any realization ${x}_{1:t}$ of states, we have
\begin{equation}\label{eq:indepen}
    \prob^{(g^1,g^2)}({x}_{1:t}|c_t)=\displaystyle\prod_{i=1}^{2} \prob^{g^i}(x^{i}_{1:t}|c_t), 
    \end{equation}
    Further, $\prob^{g^i}(x^{i}_{1:t}|c_t)$ depends only on agent $i$' strategy and not on the strategy of agent $-i$.
\end{lemma}    
\begin{proof}
This lemma is similar to Proposition 1 of \cite{mahajan2013optimal} except for the possibility of randomization in agents' strategies. A proof is provided in 
 Appendix ~\ref{proof:CI1}.
%  \red{Comment: we need to mention somewhere how our model compare to control sharing paper's model}
\end{proof}
The following theorem shows that agents can ignore their past states  without losing optimality. This allows agents to use simpler strategies where the control actions depend only on the current state and the common information.


\begin{theorem} \label{PROP:ONE}
 Agents can use symmetric strategies of the form below
\begin{equation} \label{eq:structure1}
   \delta{U}^i_t= \bar{g}_t(X^i_{t},C_t), ~~ i=1,2,
\end{equation}
without loss of optimality.  In other words, at time $t$, agent $i$ does not need its past local states, $X^i_{1:t-1}$, for making optimal decisions.
\end{theorem}
\begin{proof}
% To  prove this result, we fix agent $-i$'s strategy to an arbitrary choice and then show that agent $i$'s  decision problem can be modeled as an MDP in a suitable state space. The result then follows from the fact that Markovian strategies are optimal in an MDP.  
We provide an outline of our proof below. A detailed proof is provided in Appendix \ref{Proof_Proposition1}.

 Consider any arbitrary symmetric strategy pair $(g,g)$ for the team. To prove the theorem, it suffices to show that there is a symmetric strategy pair $(\bar{g},\bar{g})$ for the team such that, for each $t$, $\bar{g}_t$ is a function of $X_t^i,C_t$ and 
\begin{align}\label{perf:cost}
    J(\bar{g},\bar{g}) = J(g,g).
\end{align}
% \blue{Construction of g}
%\emph{for every strategy $g^2 \in \mathcal{G}^2$.}
% \blue{How to find $\bar{g}$, explain}
% \blue{why the claim works out and briefly explain}
Because of the structure of the cost function in \eqref{eq:cost2}, it is sufficient to show that for each time $t$, the joint probability distributions of $(X_t,U_t,C_t)$ under strategies $g$ and $\bar{g}$ are the same, i.e.,
\begin{align}\label{eq:joint_dist_xuc}
    \prob^{({g},{g})}[x_t,u_t,c_t] = \prob^{(\bar{g},\bar{g})}[x_t,u_t,c_t],
\end{align}
for all $x_t,u_t,c_t$. 

For $t=1$, it is straightforward to see that if we define $\bar{g}_1:={g}_1$, then \eqref{eq:joint_dist_xuc} will hold. Further, this $\bar{g}_1$ will ensure that the joint probability distribution of $(X_2,C_2)$ will be the same under $g$ and $\bar{g}$. We can now proceed inductively as follows:
Assuming that the joint probability distribution of $(X_t,C_t)$ is same under $g$ and $\bar{g}$, we will construct $\bar{g}_t$ such that \eqref{eq:joint_dist_xuc} holds and the joint distribution of $(X_{t+1},C_{t+1})$ is the same under $g$ and $\bar{g}$. To do so, we will utilise the following key fact for our setting: 
% Given the strategy profile $(g,g)$, let $\prob^{({g},{g})}[x_t,u_t,c_t]$ be the occupation measure of $[x_t,u_t,c_t]$ under strategy $g$.

\textbf{Fact 1:}
Consider any realization $x \in \mathcal{X}$, $u \in \mathcal{U}$ and $c_t \in \mathcal{U}^{t-1}$
such that $\prob^{({g},{g})}[X^1_t=x,C_t=c_t]>0$ and $\prob^{({g},{g})}[X^2_t=x,C_t=c_t]>0$. Then, the following holds:
\begin{align*}\label{eq:fact1}
  \prob^{({g},{g})}[U^1_t=u|X^1_t=x,& C_t=c_t]\notag\\
  =&\prob^{({g},{g})}[U^2_t=u|X^2_t=x,C_t=c_t].
\end{align*}
% \red{why not $C_t=c_t$ above?}
Fact 1 suggests that the conditional probability of $U^i_t$ given $X^i_t$ and $C_t$ can serve as a \emph{symmetric} strategy pair for the two agents (because of the equality in \eqref{eq:fact1}). Thus, we define the following symmetric strategy with reduced information:
\begin{align}
    \bar{g}(x,c_t;u):=\prob^{({g},{g})}[U^1_t=u|X^1_t=x,C_t=c_t],
\end{align}
for any $x \in \mathcal{X}$, $u \in \mathcal{U}$ and $c_t \in \mathcal{U}^{t-1}$
such that $\prob^{({g},{g})}[X^1_t=x,C_t=c_t]>0$ and $\prob^{({g},{g})}[X^2_t=x,C_t=c_t]>0$.
By suitably extending the definition of $\bar{g}$ for realizations where $\prob^{({g},{g})}[X^1_t=x,C_t=c_t]=0$ or $\prob^{({g},{g})}[X^2_t=x,C_t=c_t]=0$, we can show that \eqref{eq:joint_dist_xuc} holds at time $t$ and the joint probability distribution of $(X_t,U_t,C_t)$ is same under $g$ and $\bar{g}$.
\end{proof}


% we can show inductively that \eqref{eq:joint_dist_xuc} holds for all $t$.


% \begin{align}
%     \frac{\prob^{({g},{g})}[x_t,u_t,c_t]}{\prob^{({g},{g})}[x_t,c_t]}=\prob^{(g,g)}[u_t \mid x_t, c_t] \label{Outline:eqn}
% \end{align}
% where \eqref{Outline:eqn} factorizes into: 
% \begin{align*}
%   \prob^{g}[u^1_t \mid x^1_t, c_t]\prob^{g}[u^2_t \mid x^2_t, c_t]  
% \end{align*}

% and each factor $\prob^{g}[u^i_t \mid x^i_t, c_t]$ is $\bar{g}(x_t^i,c_t;u^i_t)$. This clearly is a policy which uses $x_t^i,c_t$ and using proof by induction we show that $\bar{g}$ has the same occupation measure as $g$.
% \red{Because of the structure of the total expected cost its sufficient to show that the occupation measure of both strategies are same
% 1) Given strategy (g,g), let $\prob^{({g},{g})}[x_t,u_t,c_t]$ be the Occ. measure of $[x_t,u_t,c_t]$ under strategy g.
% 2)We define $(\bar{g},\bar{g})$ as $\prob^{({g},{g})}[x_t,u_t,c_t]/\prob^{({g},{g})}[x_t,c_t]$ factorizes and each factor is $\bar{g}$ .This clearly is a policy which uses $X_t^i,C_t$ once defined carefully 
% 3)We then show by induction this $\bar{g}$ has the same occupation measure as g.


% Because of the structure of the cost function in \eqref{eq:cost2}, it is sufficient to show that for each time $t$, the random variables   $(X_t,U_t,C_t)$ have the same joint distribution under strategy profiles $({g},{g})$ and $(\bar{g},\bar{g})$. We prove this by induction. It is easy to verify that at time $t=1$, $(X_1,U_1,C_1)$ have the same joint distribution under strategy profiles $({g},{g})$ and $(\bar{g},\bar{g})$.

% Now assume that at time $t$, 
% \begin{align}
% \label{jointeq1}\prob^{({g},{g})}[x_t,u_t,c_t] = \prob^{(\bar{g},\bar{g})}[x_t,u_t,c_t],
% \end{align}
% for any realization of state, actions and common information $x_t,u_t,c_t$. Then $c_{t+1}=(c_t,u_t)$ we have
% \begin{align}
% &\prob^{({g},{g})}[x_{t+1},c_{t+1}] =\sum_{\bar{x}_t} \prob[x_{t+1}\mid {\bar{x}_t},u_t]\prob^{({g},{g})}[\bar{x}_t,u_t,c_{t}]\notag\\
% &=\sum_{\bar{x}_t}\prob[x^1_{t+1}\mid {\bar{x}^1_t},u_t]\prob[x^2_{t+1}\mid {\bar{x}^2_t},u_t]\prob^{(\bar{g},\bar{g})}[\bar{x}_t,u_t,c_{t}]\notag\\
% &=\prob^{(\bar{g},\bar{g})}[x_{t+1},c_{t+1}]\label{indhyp1}
% \end{align}
% The equality in (\ref{indhyp1}) is due to the system dynamics and induction hypothesis. Suppose at time $t$, we have
% \begin{align}\label{assumA1}
% \prob^{(g,g)}[U_t = u_t \mid X_t, C_t] = \bar{g}_t(X_t,C_{t};u_t)
% \end{align}
% almost surely for every $u_t$ (proof in Lemma \ref{aseqstrat2} of Appendix \ref{proponeproof}).
% At $t+1$, for any realization $x_{t+1},u_{t+1},c_{t+1}$ that has non-zero probability of occurrence under the strategy profile ${({g},{g})}$, we have
% \begin{align}
% \label{constarga}&\prob^{({g},{g})}[x_{t+1},u_{t+1},c_{t+1}] \\
% &= \prob^{({g},{g})}[u_{t+1}\mid x_{t+1},c_{t+1}]\prob^{({g},{g})}[x_{t+1},c_{t+1}]\\
% &= \bar{g}_t(x_{t+1},c_{t+1};u_{t+1})\prob^{(\bar{g},\bar{g})}[x_{t+1},c_{t+1}]\label{constarg11}\\
% &= \prob^{(\bar{g},\bar{g})}[u_{t+1}\mid x_{t+1},c_{t+1}]\prob^{(\bar{g},\bar{g})}[x_{t+1},c_{t+1}]\label{constarg31}\\
% &= \prob^{(\bar{g},\bar{g})}[x_{t+1},u_{t+1},c_{t+1}]\label{constarg41},
% \end{align}
% where the equality in \eqref{constarga} is a consequence of the chain rule and the manner in which players randomize their actions. Equality in \eqref{constarg11} follows from \eqref{assumA1} and the equality in \eqref{constarg3} follows from the result in \eqref{indhyp1}.
% Therefore, by induction, the equality in \eqref{jointeq1} holds for all $t$. This concludes the strategy $(\bar{g},\bar{g})$ satisfies, $J(\bar{g},\bar{g}) = J({g},{g})$.

% Suppose that the above claim is true. 
% Let $(g',g')$ be a min strategy for the team.
% Due to above claim, there exists a strategy $\bar{g}',\bar{g}'$ for the team such that, for each $t$, $\bar{g}'_t$ are functions of $X_t^i$ and $C_t$
% \[
% J(\bar{g}',\bar{g}') = J(g',g')=\inf_{g}J(g,g),
% \]

% Thus, $(\bar{g}',\bar{g}')$ is a min strategy for Team wherein Player uses only the current state and common information.



% Define the distribution $\Phi^i_t(c_t)$ over the space $\X^i_t \times \U^i_t$ as follows
% \begin{align}
% \Phi^i_t(c_t; x^i_t, u^i_t) \doteq \prob^{g}[X^i_{t},U^i_t = (x^i_{t},u^i_t) \mid C_t=c_t].\label{eq:phia}
% \end{align}
% \textbf{Example to show that $\phi^i(\cdot)$ is different for both the agents}
% Consider 

==> prob_for.tex <==
Consider a discrete-time system with two agents. Let $X^i_t \in \mathcal{X}$ denote the local state of agent $i$, $i=1,2$, at time $t$. $X_t:=(X^1_t,X^2_t)$ represents the local states of both agents at time $t$.  Each agent perfectly observes its own local state.  Let $U^i_t \in \mathcal{U}$ denote the control action of agent $i$ at time $t$. $U_t:=(U^1_t,U^2_t)$ represents the control actions of both agents at time $t$. 
 The local state of agent $i$, $i=1,2$, evolves according to 
\begin{equation}\label{eq:dyna}
    X^i_{t+1}=f_t(X^{i}_{t},U_t,W^i_t), 
\end{equation}
where $W^i_t \in \mathcal{W}$ is the random disturbance in dynamics with  probability distribution $P_{W}$. Note that the next local state of agent $i$ depends on its own current local state and the  control actions of both the agents. Also note that the function $f_t$ in \eqref{eq:dyna} is the same for both agents. The initial local states of the two agents at $t=1$, $(X^1_1, X^2_1),$ are independent random variables with $X^i_1$ having the probability distribution $P_{X_1}$. The initial states $X^1_1,X^2_1$ and the disturbances  $W^i_t, t \ge 1$, $i=1,2$, are independent random variables.

\textit{Information structure, randomization, and symmetric strategies:}
At the beginning of time $t$, agent $i$ has access to its own state history as well as the action history of both agents. Thus, the full information available to agent $i$ at time $t$  is given by 
\begin{equation}
    I^i_{t}=\{X^i_{1:t},U_{1:t-1}\}.
\end{equation}
Agent $i$ can use this information to make its control decision at time $t$. Agent $i$ is free to randomize when making its control decision. Specifically, at each time $t$, agent $i$ uses its information   to select a probability distribution $\delta{U}^i_t$ on the control space $\mathcal{U}$. That is,
\begin{equation}\label{commact}
    \delta{U}^i_t = g^i_t(I^i_{t}),
\end{equation}
where $g^i_t$ is a mapping from $\mathcal{X}^t \times \mathcal{U}^{t-1}$ to $\Delta(\mathcal{U})$.
The action  $U^i_t$ is then  randomly selected according to the chosen distribution, i.e., $U^i_t \sim \delta{U}^i_t $.
%The control stations perfectly recall all the data they observe. Thus, in the full observation model, control station $i$ chooses a communication action according to 
 The function $g^i_t$ is referred to as the control strategy of agent $i$ at time $t$.
  The collection of functions $g^i:= (g^i_1, \ldots, g^i_T)$ is referred to as the control strategy of agent $i$. Let $\mathcal{G}$ denote the set of all possible strategies for agent $i$. Note that set  of all possible strategies is the same for the two agents since they have the same  action space $\mathcal{U}$ and   state space $\mathcal{X}$.
  
  We use $(g^1,g^2)$ to denote the pair of strategies being used by agent 1 and agent 2 respectively.
 Our focus will be on the case of \emph{symmetric strategies}, i.e., the case where both agents use the same control strategy. When referring to symmetric strategies, we will drop the superscript $i$ in $g^i$  and denote a symmetric strategy pair by $(g,g)$.

\textit{Strategy optimization problem:} At time $t$, the system incurs a cost $k_t(X^1_t,X^2_t,U^1_t,U^2_t)$ that depends on the local states and control actions of both agents.
% In addition, a communication cost $\rho$ is incurred each time the agents share local states with each other.
The system runs for a time horizon $T$. The total expected cost associated with a  strategy pair $(g^1,g^2)$ is given by 
\begin{equation}\label{eq:cost2}
  J(g^1,g^2):=\ee^{(g^1,g^2)}\left[\sum_{t=1}^{T}k_t({X}_t,{U}_t)\right].
\end{equation}
% \blue{change cost $c_t$ to $k_t$}
Our objective is to find a symmetric strategy pair  that achieves the minimum total expected cost among all symmetric strategy pairs. That is, we are looking for a strategy $g \in \mathcal{G}$ such that 
\begin{equation}\label{eq:optimalg}
    J(g,g) \leq J(h,h),~ ~\forall h \in \mathcal{G}.
\end{equation}


\begin{remark}
% \red{Mention and explain independent randomization: We assume that the randomization at each agent is done independently over time and independently of the other agent. This can be done as follows:  Add a brief description of randomization along the lines of section 2.2, page 7, of this paper https://arxiv.org/pdf/1909.01445.pdf}  

\blue{We assume that the randomization at each agent is done independently over time and independently of the other agent \cite{kartik2021upper}. This can be done as follows:}
\blue{Agent $i$ has access to i.i.d. random variables $K^i_{1:T}$ that are uniformly distributed over the interval $(0, 1]$. The variables $K^1_{1:T}$, $K^2_{1:T}$ are independent of each other and of the primitive random variables. Further, agent $i$ has access to a mechanism $\kappa$ that takes as input $K^i_t$ and distribution $\delta{U}^i_t$ over $\U$ and generates a random action with the input distribution. Thus, agent $i$’s action at time t can be written as $U^i_t = \kappa(\delta{U}^i_t, K^i_t)$.}
\end{remark}

%minimizes the total cost in \eqref{eq:cost2}.

\begin{remark}
It can be shown that the strategy space $\mathcal{G}$ is a compact space and that $J(g,g)$ is a continuous function of $g \in \mathcal{G}$. Thus, an optimal $g$ satisfying \eqref{eq:optimalg} exists.
\end{remark}

\subsection{Why are randomized strategies needed?}
% \blue{Text about why randomization is required in this case}
In team problems, it is well known that randomization is not required generally \cite{yuksel2013stochastic}. However, since the agents are restricted to use symmetric strategies in our setup, randomization can help. This can be illustrated by the following simple example:
% \subsection{Example to show randomization is helpful in case of symmetric strategies:}
Let $T=1$ and the state ${X}_1 = (X^1_1, X^2_1) =(0,0)$ with probability $1$. The action space is $\mathcal{U} = \{0,1\}$. The cost at $t=1$ is given by
\begin{equation}
  k_1({X}_1,{U}_1)=\begin{cases}
    0, ~ \text{if} ~\mathds{1}_{\{u^1_{1} \neq u^2_{1}  \}}\\
    1, ~ \text{if} ~\mathds{1}_{\{u^1_{1} = u^2_{1}  \}}.
  \end{cases} \label{example_cost}
\end{equation}
Note that the cost function penalizes the agents for taking the same action.

In this case, each agent has only two \emph{deterministic} strategies -- taking action $0$ or action $1$. If both agents use the same deterministic strategy, then, clearly, $U^1_1 = U^2_1$ and hence the expected cost incurred is $1$.
% {Deterministic symmetric strategies}: 
% \begin{align}
%   (u^1_1,u^2_1)=
%   \begin{cases}
%     (g(0),g(0))=(0,0), ~ c_1({X}_1,{U}_1)= 1  \\
%     (g(0),g(0))=(1,1), ~ c_1({X}_1,{U}_1)= 1.
%   \end{cases} \label{example_cost}
% \end{align}


% The achievable deterministic symmetric strategies are $(0,0)$ \& $(1,1)$, where both the strategies incur a cost of $1$.
%The best deterministic symmetric strategy incurs control cost of $1$.
%In case of random symmetric strategies, if both agents take action $1$ with probability $p$ i.e.,
Consider now the following randomized strategy for each agent:
\begin{equation}
U^i_1= \begin{cases}
    1, ~ w.p. ~p  \\
    0, ~ w.p. ~1-p.
  \end{cases} \label{example_cost}
\end{equation}
% \textbf{Random symmetric strategies}:
When the two agents use the above randomized strategy,   the total expected cost is
$\mathds{E}[k_1({X}_1,{U}_1)]=p^2+(1-p)^2$. 
With $p=0.5$, the total expected cost of the randomized symmetric strategies described above is $0.5$ which is less than the expected cost achieved by any deterministic symmetric strategy pair. Thus, when agents are restricted to use the same strategies, they can benefit from randomization.
% The system runs for $T=1$ and sum of control costs over time horizon $T=1$ is given by $c_1({X}_1,{U}_1)=U^1_1X^1_1+U^2_1X^2_1$. Let $X^1_1=X^2_1$ and $X^1_1$ evolve as a Bernoulli random variable with probability $0.5$.
% \begin{equation}
%   X^1_1=\begin{cases}
%     1, ~ with ~probability ~0.5.\\
%     0, ~ with ~probability ~0.5.
%   \end{cases} \label{erasure_model}
% \end{equation}
% For the deterministic control strategy case, let $U^i_1=X^i_1$ and in the case of randomized control strategy, let $U^i_1$ be a Bernoulli random variable with probability $0.5$ irrespective of $X^i_1$.
% \begin{equation}
%   U^i_1=\begin{cases}
%     1, ~ with ~probability ~0.5.\\
%     0, ~ with ~probability ~0.5.
%   \end{cases} \label{erasure_model}
% \end{equation}
% \begin{itemize}
%     \item Deterministic control strategy: $\ee\left[c_1({X}_1,{U}_1)\right]=1$
%     \item Random control strategy: $\ee\left[c_1({X}_1,{U}_1)\right]=0.5$
% \end{itemize}
% The example illustrates that having a random control strategy helps in minimizing total expected control cost in the case of symmetric strategies among both the agents.

==> sagar_prob_for.tex <==
Consider a discrete-time system with two agents. Let $X^i_t \in \mathcal{X}$ denote the local state of agent $i$, $i=1,2$, at time $t$. $X_t:=(X^1_t,X^2_t)$ represents the local states of both agents at time $t$.  Each agent perfectly observes its own local state.  Let $U^i_t \in \mathcal{U}$ denote the control action of agent $i$ at time $t$. $U_t:=(U^1_t,U^2_t)$ represents the control actions of both agents at time $t$. 
 The local state of agent $i$, $i=1,2$, evolves according to 
\begin{equation}\label{eq:dyna}
    X^i_{t+1}=f_t(X^{i}_{t},U_t,W^i_t), 
\end{equation}
where $W^i_t \in \mathcal{W}$ is the random disturbance in dynamics with  probability distribution $P_{W}$. Note that the next local state of agent $i$ depends on its own current local state and the  control actions of both the agents. Also note that the function $f_t$ in \eqref{eq:dyna} is the same for both agents. The initial local states of the two agents at $t=1$, $(X^1_1, X^2_1),$ are independent random variables with $X^i_1$ having the probability distribution $P_{X_1}$. The initial states $X^1_1,X^2_1$ and the disturbances  $W^i_t, t \ge 1$, $i=1,2$, are independent random variables.

\subsection{Information structure}
% \textit{Information structure, randomization, and symmetric strategies:}
Full Information structure: At the beginning of time $t$, agent $i$ has access to its own state history as well as the action history of both agents. Thus, the full information available to agent $i$ at time $t$  is given by 
\begin{equation}
    I^i_{t}=\{X^i_{1:t},U_{1:t-1}\}.
\end{equation}
Reduced Information structure: Agents can ignore most of the information available to them without compromising the performance. At time $t$, agent $i$ can shed its state history. Thus, the reduced information available to agent $i$ at time $t$ is given by 
\begin{equation}
    I^{i,red}_{t}=\{X^i_{t},U_{1:t-1}\}.
\end{equation}
\subsection{Randomization and Symmetric strategies}
Agent $i$ can use this information to make its control decision at time $t$. Agent $i$ is free to randomize when making its control decision. Specifically, at each time $t$, agent $i$ uses its information   to select a probability distribution $\delta{U}^i_t$ on the control space $\mathcal{U}$. That is,
\begin{equation}\label{commact}
    \delta{U}^i_t = g^i_t(I^i_{t}),
\end{equation}
where $g^i_t$ is a mapping from $\mathcal{X}^t \times \mathcal{U}^{t-1}$ to $\Delta(\mathcal{U})$.
The action  $U^i_t$ is then  randomly selected according to the chosen distribution, i.e., $U^i_t \sim \delta{U}^i_t $.
%The control stations perfectly recall all the data they observe. Thus, in the full observation model, control station $i$ chooses a communication action according to 
 The function $g^i_t$ is referred to as the control strategy of agent $i$ at time $t$.
  The collection of functions $g^i:= (g^i_1, \ldots, g^i_T)$ is referred to as the control strategy of agent $i$. Let $\mathcal{G}$ denote the set of all possible strategies for agent $i$. Note that set  of all possible strategies is the same for the two agents since they have the same  action space $\mathcal{U}$ and   state space $\mathcal{X}$.
  
  We use $(g^1,g^2)$ to denote the pair of strategies being used by agent 1 and agent 2 respectively.
 Our focus will be on the case of \emph{symmetric strategies}, i.e., the case where both agents use the same control strategy. When referring to symmetric strategies, we will drop the superscript $i$ in $g^i$  and denote a symmetric strategy pair by $(g,g)$.

\textit{Strategy optimization problem:} At time $t$, the system incurs a cost $k_t(X^1_t,X^2_t,U^1_t,U^2_t)$ that depends on the local states and control actions of both agents.
% In addition, a communication cost $\rho$ is incurred each time the agents share local states with each other.
The system runs for a time horizon $T$. The total expected cost associated with a  strategy pair $(g^1,g^2)$ is given by 
\begin{equation}\label{eq:cost2}
  J(g^1,g^2):=\ee^{(g^1,g^2)}\left[\sum_{t=1}^{T}k_t({X}_t,{U}_t)\right].
\end{equation}
% \blue{change cost $c_t$ to $k_t$}
Our objective is to find a symmetric strategy pair  that achieves the minimum total expected cost among all symmetric strategy pairs. That is, we are looking for a strategy $g \in \mathcal{G}$ such that 
\begin{equation}\label{eq:optimalg}
    J(g,g) \leq J(h,h),~ ~\forall h \in \mathcal{G}.
\end{equation}


\begin{remark}
% \red{Mention and explain independent randomization: We assume that the randomization at each agent is done independently over time and independently of the other agent. This can be done as follows:  Add a brief description of randomization along the lines of section 2.2, page 7, of this paper https://arxiv.org/pdf/1909.01445.pdf}  

\blue{We assume that the randomization at each agent is done independently over time and independently of the other agent \cite{kartik2021upper}. This can be done as follows:}
\blue{Agent $i$ has access to i.i.d. random variables $K^i_{1:T}$ that are uniformly distributed over the interval $(0, 1]$. The variables $K^1_{1:T}$, $K^2_{1:T}$ are independent of each other and of the primitive random variables. Further, agent $i$ has access to a mechanism $\kappa$ that takes as input $K^i_t$ and distribution $\delta{U}^i_t$ over $\U$ and generates a random action with the input distribution. Thus, agent $i$’s action at time t can be written as $U^i_t = \kappa(\delta{U}^i_t, K^i_t)$.}
\end{remark}

%minimizes the total cost in \eqref{eq:cost2}.

\begin{remark}
It can be shown that the strategy space $\mathcal{G}$ is a compact space and that $J(g,g)$ is a continuous function of $g \in \mathcal{G}$. Thus, an optimal $g$ satisfying \eqref{eq:optimalg} exists.
\end{remark}

\subsection{Why are randomized strategies needed?}
% \blue{Text about why randomization is required in this case}
In team problems, it is well known that randomization is not required generally \cite{yuksel2013stochastic}. However, since the agents are restricted to use symmetric strategies in our setup, randomization can help. This can be illustrated by the following simple example:
% \subsection{Example to show randomization is helpful in case of symmetric strategies:}
Let $T=1$ and the state ${X}_1 = (X^1_1, X^2_1) =(0,0)$ with probability $1$. The action space is $\mathcal{U} = \{0,1\}$. The cost at $t=1$ is given by
\begin{equation}
  k_1({X}_1,{U}_1)=\begin{cases}
    0, ~ \text{if} ~\mathds{1}_{\{u^1_{1} \neq u^2_{1}  \}}\\
    1, ~ \text{if} ~\mathds{1}_{\{u^1_{1} = u^2_{1}  \}}.
  \end{cases} \label{example_cost}
\end{equation}
Note that the cost function penalizes the agents for taking the same action.

In this case, each agent has only two \emph{deterministic} strategies -- taking action $0$ or action $1$. If both agents use the same deterministic strategy, then, clearly, $U^1_1 = U^2_1$ and hence the expected cost incurred is $1$.
% {Deterministic symmetric strategies}: 
% \begin{align}
%   (u^1_1,u^2_1)=
%   \begin{cases}
%     (g(0),g(0))=(0,0), ~ c_1({X}_1,{U}_1)= 1  \\
%     (g(0),g(0))=(1,1), ~ c_1({X}_1,{U}_1)= 1.
%   \end{cases} \label{example_cost}
% \end{align}


% The achievable deterministic symmetric strategies are $(0,0)$ \& $(1,1)$, where both the strategies incur a cost of $1$.
%The best deterministic symmetric strategy incurs control cost of $1$.
%In case of random symmetric strategies, if both agents take action $1$ with probability $p$ i.e.,
Consider now the following randomized strategy for each agent:
\begin{equation}
U^i_1= \begin{cases}
    1, ~ w.p. ~p  \\
    0, ~ w.p. ~1-p.
  \end{cases} \label{example_cost}
\end{equation}
% \textbf{Random symmetric strategies}:
When the two agents use the above randomized strategy,   the total expected cost is
$\mathds{E}[k_1({X}_1,{U}_1)]=p^2+(1-p)^2$. 
With $p=0.5$, the total expected cost of the randomized symmetric strategies described above is $0.5$ which is less than the expected cost achieved by any deterministic symmetric strategy pair. Thus, when agents are restricted to use the same strategies, they can benefit from randomization.
% The system runs for $T=1$ and sum of control costs over time horizon $T=1$ is given by $c_1({X}_1,{U}_1)=U^1_1X^1_1+U^2_1X^2_1$. Let $X^1_1=X^2_1$ and $X^1_1$ evolve as a Bernoulli random variable with probability $0.5$.
% \begin{equation}
%   X^1_1=\begin{cases}
%     1, ~ with ~probability ~0.5.\\
%     0, ~ with ~probability ~0.5.
%   \end{cases} \label{erasure_model}
% \end{equation}
% For the deterministic control strategy case, let $U^i_1=X^i_1$ and in the case of randomized control strategy, let $U^i_1$ be a Bernoulli random variable with probability $0.5$ irrespective of $X^i_1$.
% \begin{equation}
%   U^i_1=\begin{cases}
%     1, ~ with ~probability ~0.5.\\
%     0, ~ with ~probability ~0.5.
%   \end{cases} \label{erasure_model}
% \end{equation}
% \begin{itemize}
%     \item Deterministic control strategy: $\ee\left[c_1({X}_1,{U}_1)\right]=1$
%     \item Random control strategy: $\ee\left[c_1({X}_1,{U}_1)\right]=0.5$
% \end{itemize}
% The example illustrates that having a random control strategy helps in minimizing total expected control cost in the case of symmetric strategies among both the agents.
\subsection{Reduced Information structure}
In most of the earlier works related to asymmetrical strategy pair, agents ignore lot of information available to them without compromising the performance achievable under asymmetric strategies. To do so, split the information available to the agents into two parts -- common information (which is available to both agents) and private information (which is available to only one agent). 
At time  $t$, the common information is defined as 
\begin{align}
C_t:=U_{1:t-1},\label{commoninfo}
\end{align}
and the private information for agent $i$, $i=1,2,$ is defined as 
\begin{align}
P_t^i &:= I_t^i \setminus C_t  = X^i_{1:t}.
\end{align}
In asymmetrical strategy pair, agents reduce private information without compromising the performance.
One approach for reducing private information that has been commonly used in prior literature on multi-agent/decentralized systems is called the agent-by-agent (or person-by-person approach). 
This approach works as follows: We start by fixing agent $-i$'s strategy to an arbitrary choice and then show that agent $i$ can make decisions based on a subset or a function of its private information without compromising performance. If this reduction in agent $i$'s information holds for any arbitrary strategy of agent $-i$, we can conclude that this reduction would hold for globally optimal strategy as well.  The problem with this approach, however, is that it cannot accommodate the restriction to symmetric strategies. The approach allows agents to use different strategies and the only conclusion it can make is that agents can use strategies with reduced information but these reduced-information strategies may or may not be symmetric. Thus, we cannot adopt this approach for reducing agents' private information in our problem.

Another constructive approach for reducing private information is for \emph{any given pair of strategies}, we will construct another pair of strategies with the \emph{same performance and reduced private information}. It then follows that agents can be restricted to use strategies with reduced private information without compromising performance. 
For this particular approach we consider any arbitrary strategy pair $(g^1,g^2)$ for the team. To prove the above statement, it suffices to show that there is a strategy pair $(\bar{g}^1,\bar{g}^2)$ for the team such that, for each $t$, $\bar{g}^i_t$ is a function of $X_t^i,C_t$ and 
\begin{align}\label{perf:cost}
    J(\bar{g}^1,\bar{g}^2) = J(g^1,g^2).
\end{align}
% \blue{Construction of g}
%\emph{for every strategy $g^2 \in \mathcal{G}^2$.}
% \blue{How to find $\bar{g}$, explain}
% \blue{why the claim works out and briefly explain}
Because of the structure of the cost function in \eqref{eq:cost2}, it is sufficient to show that for each time $t$, the joint probability distributions of $(X_t,U_t,C_t)$ under strategies $(g^1,g^2)$ and $(\bar{g}^1,\bar{g}^2)$ are the same, i.e.,
\begin{align}\label{eq:joint_dist_xuc1}
    \prob^{({g}^1,{g}^2)}[x_t,u_t,c_t] = \prob^{(\bar{g}^1,\bar{g}^2)}[x_t,u_t,c_t],
\end{align}
for all $x_t,u_t,c_t$. 


The challenge with this approach is that it cannot accommodate restriction to symmetric strategies. 
To prove \eqref{eq:joint_dist_xuc1}, the following key fact is used: 
% Given the strategy profile $(g,g)$, let $\prob^{({g},{g})}[x_t,u_t,c_t]$ be the occupation measure of $[x_t,u_t,c_t]$ under strategy $g$.

\textbf{Fact 1:}
Consider any realization $x \in \mathcal{X}$, $u \in \mathcal{U}$ and $c_t \in \mathcal{U}^{t-1}$
such that $\prob^{({g}^1,{g}^2)}[X^1_t=x,C_t=c_t]>0$ and $\prob^{({g}^1,{g}^2)}[X^2_t=x,C_t=c_t]>0$. Then, the following needs to be true:
\begin{align}\label{eq:fact11}
  \prob^{({g}^1,{g}^2)}[U^1_t=u|&X^1_t=x, C_t=c_t]\notag\\
  =&\prob^{({g}^1,{g}^2)}[U^2_t=u|X^2_t=x,C_t=c_t].
\end{align}
Fact 1 suggests that the conditional probability of $U^i_t$ given $X^i_t$ and $C_t$ can serve as a \emph{symmetric} strategy pair for the two agents (if equality in \eqref{eq:fact11} holds for symmetric strategy pair). We show by counter-example that \eqref{eq:fact11} does not hold true in the case of symmetric strategies.

\textbf{Counter-example}:Let the state space be $\mathcal{X} = \{0,1\}$ and action space, $\mathcal{U} = \{a,b\}$ and the states are iid. At time $t=1$,  $X^i_1 \sim {\rm Bernoulli}(1/2)$ and $X^i_2 \sim {\rm Bernoulli}(1/2)$ for any history of past state and actions, $i=1,2$. We define strategy at time, $t=1$ as follows:

\begin{equation}
g_1(u^i_1=a|x^i_1)=
 \begin{cases}
    \alpha, ~ \text{if} ~\&~ x^i_1=0\\
    \beta, ~ \text{if} ~\&~ x^i_1=1.
  \end{cases} \label{strategy2}
\end{equation}
The strategy at time $t=2$ with available full information $(x^i_2, x^i_1, u^1_1, u^2_1)$ for agent $i$ is defined as follows:

\begin{equation}
g_2(u^i_2=a|x^i_1,x^i_2,u^1_1,u^2_1)=
 \begin{cases}
    \alpha, ~ \text{if} ~\&~ x^i_1=x^i_2\\
    \beta, ~ \text{if} ~\&~ x^i_1\neq x^i_2.
  \end{cases} \label{strategy2}
\end{equation}
The reduced information strategy at time $t=2$ for realizations $(u^1_1, u^2_1)=(a,b)$ and $x^i_2=0$ is given by:
\begin{align}
    g_2(u^i_2=a|x^i_2,u^1_1,u^2_1)=\prob^g(u^i_2=a|x^i_2=0,u^1_1=a,u^2_1=b)
\end{align}
\subsubsection{Reduced information strategy for Agent 1}
\begin{align}
    &\prob^{(g,g)}(U^1_2=a|X^1_2=0,U^1_1=a,U^2_1=b)=\notag\\
    &\prob^{(g,g)}(U^1_2=a,X^1_1=0|X^1_2=0,U^1_1=a,U^2_1=b)+\notag\\
    &\prob^{(g,g)}(U^1_2=a,X^1_1=1|X^1_2=0,U^1_1=a,U^2_1=b)\notag\\
    &=\alpha \prob^{(g,g)}(X^1_1=0|X^1_2=0,U^1_1=a,U^2_1=b) \notag\\
    &+ \beta \prob^{(g,g)}(X^1_1=1|X^1_2=0,U^1_1=a,U^2_1=b)\notag\\
    &=\alpha (\frac{\alpha}{\alpha+\beta}) + \beta (\frac{\beta}{\alpha+\beta})=\frac{\alpha^2+\beta^2}{\alpha+\beta}
\end{align}

\subsubsection{Reduced information strategy for Agent 2}
\begin{align}
    &\prob^{(g,g)}(U^2_2=a|X^2_2=0,U^1_1=a,U^2_1=b)=\notag\\
    &\prob^{(g,g)}(U^2_2=a,X^2_1=0|X^2_2=0,U^1_1=a,U^2_1=b)+\notag\\
    &\prob^{(g,g)}(U^2_2=a,X^2_1=1|X^2_2=0,U^1_1=a,U^2_1=b)\notag\\
    &=\alpha \prob^{(g,g)}(X^2_1=0|X^2_2=0,U^1_1=a,U^2_1=b) \notag\\
    &+ \beta \prob^{(g,g)}(X^2_1=1|X^2_2=0,U^1_1=a,U^2_1=b)\notag\\
    &=\alpha (\frac{1-\alpha}{2-\alpha-\beta}) + \beta (\frac{1-\beta}{2-\alpha-\beta})\notag\\
    &=\frac{\alpha+\beta-\alpha^2-\beta^2}{2-\alpha-\beta}
\end{align}
for $\alpha=1/4$ and $\beta=1/2$, 
\begin{align}
    &\prob^{(g,g)}(U^1_2=a|X^1_2=0,U^1_1=a,U^2_1=b)=5/12 \notag\\
    &\prob^{(g,g)}(U^2_2=a|X^2_2=0,U^1_1=a,U^2_1=b)=7/20
\end{align}
% \begin{align}
%     \bar{g}(x,c_t;u):=\prob^{({g},{g})}[U^1_t=u|X^1_t=x,C_t=c_t],
% \end{align}
Therefore \eqref{eq:fact11} doesn't hold true for symmetric strategies.


A key conditional independence property established in the following lemma.
\begin{lemma}[Conditional independence property] \label{LEM:INDEPEN}
Consider any arbitrary (symmetric or asymmetric) choice of agents' strategies. Then, at any time $t$, the two agents'  local states are conditionally independent given the common information $C_t$. That is, if $c_t$ is the realization of the common information at time $t$ then for any realization ${x}_{1:t}$ of states, we have
\begin{equation}\label{eq:indepen}
    \prob^{(g^1,g^2)}({x}_{1:t}|c_t)=\displaystyle\prod_{i=1}^{2} \prob^{g^i}(x^{i}_{1:t}|c_t), 
    \end{equation}
    Further, $\prob^{g^i}(x^{i}_{1:t}|c_t)$ depends only on agent $i$' strategy and not on the strategy of agent $-i$.
\end{lemma}    
\begin{proof}
This lemma is similar to Proposition 1 of \cite{mahajan2013optimal} except for the possibility of randomization in agents' strategies. A proof is provided in 
 Appendix ~\ref{proof:CI1}.
%  \red{Comment: we need to mention somewhere how our model compare to control sharing paper's model}
\end{proof}

==> simulation.tex <==
%% Add simulation section in this file
%\section{Simulations} 
In this section, {we illustrate the performance of \texttt{TSDE-MF} for a
homogeneous (i.e., $|M| = 1$) mean-field LQ system for different values of
the number $n$ of agents, with $\MAT A=1,\MAT B=0.3,\MAT D=0.5,\MAT E=0.2, \MAT Q=1,\bar{\MAT Q}=1, \MAT R=1$,and $\bar{\MAT R}=0.5$. We set the local noise variance $\sigma_w^2=1$. } 

{For the regret plots in Figure \ref{fig:regreta},\ref{fig:regretb}, we set the common noise variance to $\sigma_v^2+\sigma_{v^0}^2=1$. 
The prior distribution used in the simulation are set according to \textbf{(A3)} and \textbf{(A4)} with $\breve \mu(\ell)=[1,1]$, $\bar \mu(\ell)=[1,1]$, $\bar{\Sigma}_1=I$, and $\breve{\Sigma}_1=I$, $\breve\Theta = \{\breve{\theta}: \MAT A + \MAT B  \breve {\MAT L}(\breve \theta) \leq \delta \}$, $\bar\Theta = \{\bar{\theta}: \MAT A + \MAT D + (\MAT B+\MAT E) \bar{\MAT L}(\bar \theta) \leq \delta \}$ and $\delta = 0.99$. }

{In the comparison of {\tt TSDE-MF} method with {\tt TSDE} in Figure \ref{fig:regretc}, we consider the same dynamics and cost parameters as above but without common noise (i.e. $\sigma_v^2+\sigma_{v^0}^2=0$).}
%See supplementary file of \cite{gagrani2020thompson} for the choice of parameters.

\paragraph{Empirical evaluation of regret:}

We run the system for $500$ different sample paths and plot the mean and
standard deviation of the expected regret $R(T)$ for $T = 5000$. The regret
for different values of $n$ is shown in~\ref{fig:regreta}--\ref{fig:regretb}. As seen from the
plots, the regret reduces with the number of agents and $R(T)/\sqrt{T}$
converges to a constant. Thus, the empirical regret matches the upper bound of
$\tilde{\mathcal{O}}( (1 + \frac1n)\sqrt{T})$ obtained in Theorem~\ref{thm:main}. 

\paragraph{Comparison with naive TSDE algorithm:}
We compare the performance of \texttt{TSDE-MF} with that of directly using the \texttt{TSDE}
algorithm presented in \cite{ouyang2017control,ouyang2019posterior} for
different values of $n$. The results are shown in Fig.~\ref{fig:regretc}. As
seen from the plots, the regret of \texttt{TSDE-MF} is smaller than
\texttt{TSDE} but more importantly, the regret of \texttt{TSDE-MF} reduces
with $n$ while that of \texttt{TSDE} increases with $n$. This matches their
respective upper bounds of $\tilde{\mathcal{O}}( (1 + \frac1n) \sqrt{T})$ and
$\tilde{\mathcal{O}}(n^{1.5} \sqrt{T})$. These plots clearly illustrate the
significance of our results even for small values of~$n$.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.45\linewidth]{plot3}
%     \caption{Comparison of \texttt{TSDE-MF} and \texttt{TSDE}.} 
%     \label{fig:naive}
% \end{figure}



==> special_cost.tex <==
% \red{write about the prescription space in both the problems}
% The private space in problem P1b is $\mathcal{X}^{1:t}$ and the private space in problem P1c is $\mathcal{X}^{t}$. 
In Problem P1b the prescription space $\mathcal{B}_t$ is the space of functions from $\mathcal{X}^{1:t}$ to $\Delta(\mathcal{U})$ and in Problem P1c the prescription space $\mathcal{B}_t$ is the space of functions from $\mathcal{X}$ to $\Delta(\mathcal{U})$.
At time $t$, we assume that the system incurs a non negative cost $k_t(X^0_t,X^1_t,X^2_t,U^1_t,U^2_t)$.
% $c(x^1,x^2,u^1,u^2)\ge 0$ \\
% for each $x^i$ there is $m(x^i)$ such that $c(x^1,x^2,m(x^1),m(x^2))=0$
Further we assume that for each local state $x^i$ of agent $i$ there exists an action $m(x^i)$ such that the cost,  $k(x^0,x^1,x^2,m(x^1),m(x^2))=0$. 

In connection to this, we show that there is an optimal prescription in the full local history information structure problem (P1b) which belongs to the prescription space of the reduced history information structure problem (P1c). Using Dynamic program in Theorem 1, we show that $m$ is an optimal prescription in problem P1b.
% To show that the optimal strategy for Problem P1b is also optimal for P1c in this case, we consider the coordinator's dynamic program for problem P1b.
% % and show optimal prescription exists for full local history information structure. 
% Optimal prescription in the full local history information structure is also the optimal prescription in the reduced history information structure problem (P1c), because of the rich state space present in problem P1b. Let $\mathcal{{B}}$ be the space of functions from $\mathcal{X}^{1:t}$ to $\Delta(\mathcal{U})$. For a $\gamma \in \mathcal{{B}}$ and $x_{1:t} \in \mathcal{X}^{1:t}$, $\gamma(x_{1:t})$ is a probability distribution on $\mathcal{U}$.  Let $\gamma(x_{1:t};u)$ denote the probability assigned to $u \in \mathcal{U}$ under the probability distribution $\gamma(x_{1:t})$.
% \red{rewording required}

\begin{theorem}\label{thm:dpcost}
The value functions  for the coordinator's dynamic program are as follows: Define $V_{T+1}(\pi^1_{T+1},\pi^2_{T+1},x^0_{T+1}) =0$ for every $\pi^1_{T+1},\pi^2_{T+1},x^0_{T+1}$. For $t \leq T$ and  for any realization $\pi^1_{t},\pi^2_{t},x^0_{t}$ of $\Pi^1_{t},\Pi^2_{t},X^0_{t}$, define the value function $V_t(\cdot)$ and function $Q_t(\cdot)$ as follows:
% For $t\le T$, let the value function $V_t(\cdot)$ and function $Q_t(\cdot)$ be defined as follows:
 \begin{align}
    V_{t}(\pi^1_{t}&,\pi^2_{t},x^0_{t}) :=\min_{\gamma_{t} \in \mathcal{B}_t}Q_{{t}}(\pi^1_{t},\pi^2_{t},x^0_{t},\gamma_{t}) \label{eq:qfun_cost}
  \end{align}
 The non-negative $Q$ function evaluated at prescription $m$ is zero ($Q_{{t}}(\pi^1_{t},\pi^2_{t},x^0_{t},m)=0$) for any realization $\pi^1_t,\pi^2_t,x^0_t$ of $\Pi^1_t,\Pi^2_t,X^0_t$ respectively.
  Therefore,
  \begin{align}
      &Q_{{t}}(\pi^1_{t},\pi^2_{t},x^0_{t},\gamma_{t})\ge Q_{{t}}(\pi^1_{t},\pi^2_{t},x^0_{t},m),
\end{align}
for any realization $\pi^1_t,\pi^2_t,x^0_t$ of $\Pi^1_t,\Pi^2_t,X^0_t$ respectively, $V_{t}(\pi^1_{t},\pi^2_{t},x^0_{t})=0$.
The coordinator's optimal prescription is $m$ for each time.
\end{theorem}
\begin{proof}
See Appendix F.
\end{proof}
% \begin{theorem}\label{thm:dp}
% The value functions  for the coordinator's dynamic program are as follows: for any realization $\pi^1_t,\pi^2_t,x^0_t$ of $\Pi^1_t,\Pi^2_t,X^0_t$ respectively, define
The coordinator's strategy $u^i_t=m(x^i_t)$ is the optimal strategy in problem P1b and the optimal strategy is feasible in the reduced information structure problem P1c. Hence the optimal strategy is the same in both the problems.













%  \begin{align}
%   V_{T}(\pi^1_T,\pi^2_T,x^0_T) :=&\min_{\gamma_T \in \mathcal{{B}}}Q_{T}(\pi^1_T,\pi^2_T,x^0_T,\gamma_T)\notag\\
%   Q_{T}(\pi^1_T,\pi^2_T,x^0_T,\gamma_T):=&\sum_{x_{1:T}}\sum_{u_T} k_T(x_T,u_T)\pi^1_T(x^{1}_{1:T})\pi^2_T(x^{2}_{1:T}) \notag\\
%   &\times \delta_{x^0_T}(x^0) \gamma_T(x^{1}_{1:T};u^1_T)\gamma_T(x^{2}_{1:T};u^2_T)
%  \end{align}
%  $Q_{T}(\pi^1_T,\pi^2_T,x^0_T,\gamma_T)\ge 0$ for any realization $\pi^1_T,\pi^2_T,x^0_T$ of $\Pi^1_T,\Pi^2_T,X^0_T$ respectively.
% The deterministic strategy $m$ is a special case of $\gamma \in \mathcal{{B}}$, where $m(x^{i}_{1:T};u^i_T)=1$.
% \begin{align}
%     &Q_{T}(\pi^1_T,\pi^2_T,x^0_T,m):=\notag\\
%     &\sum_{x_{1:T}}\sum_{u_T} k_T(x_T,m(x^1_T),m(x^2_T))\pi^1_T(x^{1}_{1:T})\pi^2_T(x^{2}_{1:T})\delta_{x^0_T}(x^0) \notag\\
%     &=0. \label{special_cost:DP1}
% \end{align}
% Equation \eqref{special_cost:DP1} arises because of the cost, $k_T(x_T,m(x^1_T),m(x^2_T))=0$.
% \begin{align}
%     &Q_{T}(\pi^1_T,\pi^2_T,x^0_T,\gamma_T)\ge Q_{T}(\pi^1_T,\pi^2_T,x^0_T,m)=0.
%   \end{align} 
% for any realization $\pi^1_T,\pi^2_T,x^0_T$ of $\Pi^1_T,\Pi^2_T,X^0_T$ respectively.   
%   \begin{align}
%     &V_{T}(\pi^1_T,\pi^2_T,x^0_T) :=\min_{\gamma_T \in \mathcal{{B}}}Q_{T}(\pi^1_T,\pi^2_T,x^0_T,\gamma_T)=0. \label{eq:value_spec}
% \end{align} 
%  At $t=T-1$,
%  \begin{align}
%     V_{T-1}(\pi^1_{T-1}&,\pi^2_{T-1},x^0_{T-1}) :=\notag\\
%   &\min_{\gamma_{T-1} \in \mathcal{{B}}}Q_{{T-1}}(\pi^1_{T-1},\pi^2_{T-1},x^0_{T-1},\gamma_{T-1}) \label{eq:qfun_cost}
%   \end{align}
%   \begin{align}
%   &Q_{T-1}(\pi^1_{T-1},\pi^2_{T-1},x^0_{T-1},\gamma_{T-1}):=\sum_{x_{1:{T-1}}}\sum_{u_{T-1}}\pi^1_{T-1}(x^{1}_{1:{T-1}})\notag\\
%   &\times\pi^2_t(x^{2}_{1:{T-1}})\delta_{x^0_{T-1}}(x^0)\gamma_t(x^{1}_{1:{T-1}};u^1_{T-1})\gamma_t(x^{2}_{1:{T-1}};u^2_{T-1})\notag\\
%     &\times[k_{T-1}(x_{T-1},u_{T-1})+V_{T}(\pi^1_{T},\pi^2_T,x^0_T)]
%  \end{align}
%  Using equation \eqref{eq:value_spec}, $V_{T}(\pi^1_{T},\pi^2_T,x^0_T)=0$.
%  \begin{align}
%   &Q_{T-1}(\pi^1_{T-1},\pi^2_{T-1},x^0_{T-1},\gamma_{T-1}):=\notag\\
%   &\sum_{x_{1:{T-1}}}\sum_{u_{T-1}}\pi^1_{T-1}(x^{1}_{1:{T-1}})\pi^2_t(x^{2}_{1:{T-1}})\gamma_t(x^{1}_{1:{T-1}};u^1_{T-1})\notag\\
%     &\times\delta_{x^0_{T-1}}(x^0)\gamma_t(x^{2}_{1:{T-1}};u^2_{T-1})[k_{T-1}(x_{T-1},u_{T-1})]
%  \end{align}
%  $Q_{T-1}(\pi^1_{T-1},\pi^2_{T-1},x^0_{T-1},m)=0$, since the cost function $k_T(x_{T-1},m(x^1_{T-1}),m(x^2_{T-1}))=0$ from problem cost definition.
%  Therefore from equation \eqref{eq:qfun_cost}, $V_{T-1}(\pi^1_{T-1},\pi^2_{T-1},x^0_{T-1})=0$. 
%\end{theorem}
 

%   V_{T}(\beta^1_{T-1}( \pi^1_{{T-1}},\gamma_{T-1},u_{T-1}),\beta^2_{T-1}( \pi^2_{T-1},\gamma_{T-1},u_{T-1}))

%  The coordinator's optimal strategy is to pick the minimizing prescription pairs for each time and each $(\pi^1_t,\pi^2_t)$.




==> special_dynamics.tex <==
The dynamics of the global and local states in the specialized dynamics problem are as follows:
 \begin{equation}\label{eq:dyna_global2}
    X^0_{t+1} =f^0_t(X^0_t, U_t, W^0_t),
 \end{equation}
\begin{equation}\label{eq:dyna2}
    X^i_{t+1}=f_t(X^0_t, U_t,W^i_t),~~ i=1,2. 
\end{equation}
The global and local state dynamics are similar to \eqref{eq:dyna_global} and \eqref{eq:dyna}, except that in local dynamics the next local state doesn't depend on the current local state. To show equivalence between Problems P1b and P1c in terms of optimal cost, it is sufficient to show equivalence between Problems P1a and P1c. Using Lemma 1, equivalence between Problems P1a and P1c implies equivalence between Problems P1b and P1c in terms of optimal cost. To prove equivalence between Problems P1a and P1c, we show that the coordinator's dynamic program are identical in both cases.

Towards this we show that the coordinator belief is the same for both problems in the following lemma.
\begin{lemma}\label{LEM:UPDATEspecdyn}
For $i=1,2$ and for each $t \geq 1$, if $x^0_t,u_t$ is the realization of global state($X^0_t$) and action($U_t$). The coordinator's belief for all $x^i_{t+1} \in \mathcal{X}$ in problem P1a and P1c are the same and given as follows:
\begin{align}
    \Pi^{i,a}_{t+1}(x^i_{t+1})=\Pi^{i,c}_{t+1}(x^i_{t+1})=\prob(f_t(x^0_t,u_t,W^i_t)=x^i_{t+1}).
    %\prob(f_t(x^0_t,u_t,W^i_t)=x^i_{t+1}).
\end{align}
\end{lemma}
\begin{proof}
See Appendix \ref{App:lemma_special_dyn} 
% \red{say something about realizations of $X^0_t,U_t$.}
\end{proof}
\begin{lemma}\label{LEM:UPDATEspecdyn}
Suppose at time t the global state is $x^0_t$ and the beliefs on the local states are $\pi^1_t,\pi^2_t$ in both problems P1a and P1c.
Let $z^a_{t+1}:=(x^0_{t+1},u_t,x^{1,2}_t)$ be the increment in common information in problem P1a and $z^c_{t+1}:=(x^0_{t+1},u_t)$ be the increment in common information in problem P1c. Then the beliefs at time $t+1$ in the two problems are the same and given as follows:
\begin{align}
    \pi^i_{t+1}=\hat{\eta}^i_t(x^0_t,u_t)
\end{align}
where $\hat{\eta}^i_t(x^0_t,u_t)$ is the probability distribution of $f_t(x^0_t,u_t,W^i_t)$.
\end{lemma}
% \red{The beliefs are the same for all time $t$.}
At time $t=1$, the beliefs are the same for both problems and the above lemma proves that the beliefs are same for all time $t$.
% Lemma \ref{LEM:UPDATEspecdyn} implies that the belief for Problem P1a and P1c are the same for all time, $t \geq 1$ and for all $x^i \in \mathcal{X}$.
% \begin{itemize}
%     \item Dynamic program of P1a and P1c are the same.
%     \item Towards this we show that the belief update is the same.(lemma to show that)
%     \item 1-2 sentences explaining why value functions are the same.
%     \item Everything in the value function is the same by comparing it with t+1 and prescription space is the same.
%     \item the optimal cost in each problem is the exp of $V_1$ evaluated at prior belief and $X^0_1$, value fns are the same implies optimal cost J are the same..
% \end{itemize}

Recall that the private information $p=x$ are same for both the problems, therefore this leads to same prescription space $B_t$.
The Dynamic program in Theorem \ref{thm:dp} when applied to problem P1a and P1c are as follows:
\begin{corollary}\label{thm:dpspecial_dyna}
Define $V^a_{T+1}(x^0_{t+1},\pi^1_{T+1},\pi^2_{T+1}) =0$ and $V^c_{T+1}(x^0_{t+1},\pi^1_{T+1},\pi^2_{T+1}) =0$ for every $x^0_{t+1},\pi^1_{T+1},\pi^2_{T+1}$. For $t \leq T$ and  for any realization $x^0_{t},\pi^1_{t},\pi^2_{t}$ of $X^0_{t},\Pi^1_{t},\Pi^2_{t}$, define
\begin{align}
    &V^a_t(x^0_{t},\pi^1_{t},\pi^2_{t}) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}[k_t(X_t, U_t) +V^a_{t+1}(\delta_{X^0_{t+1}}, \\ \notag 
    &\hat{\eta}^1_t(x^0_t,U_t),\hat{\eta}^2_t(x^0_t,U_t)) |(X^0_{t},\Pi^1_{t},\Pi^2_{t},\Gamma_t)=(x^0_{t},\pi^1_{t},\pi^2_{t},\gamma_t)]\label{eq:DP1}
\end{align}
\begin{align}
    &V^c_t(x^0_{t},\pi^1_{t},\pi^2_{t}) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}[k_t(X_t, U_t) +V^c_{t+1}(\delta_{X^0_{t+1}}, \\ \notag 
    &\hat{\eta}^1_t(x^0_t,U_t),\hat{\eta}^2_t(x^0_t,U_t)) |(X^0_{t},\Pi^1_{t},\Pi^2_{t},\Gamma_t)=(x^0_{t},\pi^1_{t},\pi^2_{t},\gamma_t)]\label{eq:DP2}
\end{align}
\end{corollary}
% \begin{corollary}\label{thm:dpspecial_dyna}
% Define $V^a_{T+1}(\pi_{T+1}) =0$ and $V^c_{T+1}(\pi_{T+1}) =0$ for every $\pi_{T+1}$. For $t \leq T$ and  for any realization $\pi_{t}$ of $\Pi_{t}$, define
% \begin{align}
%     V^a_t(\pi_{t}) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}&[k_t(X_t, U_t) +\\ \notag 
%     &V^a_{t+1}(\hat{\eta}_t(x^0_t,U_t)) |\Pi_{t}=\pi_{t},\Gamma_t=\gamma_t]\label{eq:DP1}
% \end{align}
% \begin{align}
%     V^c_t(\pi_{t}) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}&[k_t(X_t, U_t) +\\ \notag 
%     &V^c_{t+1}(\hat{\eta}_t(x^0_t,U_t)) |\Pi_{t}=\pi_{t},\Gamma_t=\gamma_t]\label{eq:DP1}
% \end{align}
% \end{corollary}
% Using Theorem 1, we can write a dynamic program for the coordinator's problem P1a and P1c.
% Using  the results in \cite{nayyar2013decentralized}, we can write a dynamic program for the coordinator's problem P1a and P1c. Recall that prescription space $\mathcal{B}_t$, is the space of all functions from $\mathcal{X}$ to $\Delta(\mathcal{U})$ and are same for problems P1a and P1c. For a $\gamma \in \mathcal{B}_t$ and $x \in \mathcal{X}$, $\gamma(x)$ is a probability distribution on $\mathcal{U}$. Let $\gamma(x;u)$ denote the probability assigned to $u \in \mathcal{U}$ under the probability distribution $\gamma(x)$. \red{make change to P=X}
Using the above Corollary, we show that in both the problems value functions are the same for any $\pi \in \delta(x)$.
 \begin{lemma}
  For $t\le T$, let $V^a_{t}(\cdot)$ be the value function for the coordinator's dynamic program in problem P1a and $V^c_{t}(\cdot)$ be the value function for the coordinator's dynamic program in  problem P1c. We show that $V^a_{t}(\pi)=V^c_{t}(\pi)$ for any $\pi \in \delta(x)$.   
 \end{lemma}
 \begin{proof}
%  \red{joint distribution of $X_t,U_t$ are the same in both problems}
 By definition value functions for both problems at time $T+1$ are same (equal to $0$). At time $T$, the value functions evaluated at the same belief leads to $(X_T,U_T)$ has a pair having the same probability distribution. Therefore, the expectations are the same and the minimization is over identical prescription space proves that the value functions are the same in both the problems.
 So using the above argument inductively backwards in time. At any time $t$, the expectation over the cost function are same in both problems because $(X_t,U_t)$ has a pair have the same probability distribution when evaluated over the same belief. Using Lemma \ref{LEM:UPDATEspecdyn}, the beliefs at time $t+1$ in the two problems are the same and from the inductive step value functions evaluated at same belief are equal.
Hence the expectations are the same and minimization over identical prescription space proves that the value functions are same for both the problems.
% By definition value functions for both problems at time $T+1$ are same for any realization $\pi^a_t$ of $\Pi^a_t$ and $\pi^c_t$ of $\Pi^c_t$. At time $T$, the terms inside the expectation are identical for both problems and the minimization is over identical prescription space. Therefore, value functions are same for both the problems at time $T$.
% So using the above argument inductively backwards in time, we show that the value functions are same for $t\le T$.
 \end{proof}
  % \red {change it to a lemma and remove the corollary}
% \begin{corollary}\label{thm:dpspecial_dyna}
% The value functions  for the coordinator's dynamic program in problem P1a and P1c are as follows: Define $V^a_{T+1}(\pi_{T+1}) =0$ and $V^c_{T+1}(\pi_{T+1}) =0$ for every $\pi_{T+1}$. For $t \leq T$ and  for any realization $\pi_t$ of $\Pi_t$, define
% \begin{align}
%     V^a_t&(\pi_t) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}[k_t(X_t, U_t) + \\ \notag 
%         &V^a_{t+1}(\delta_{X^0_t}(x^0),\hat{\eta}^1_t(x^0_t,u_t),\hat{\eta}^2_t(x^0_t,u_t)) | \Pi_t = \pi_t, \Gamma_t = \gamma_t]\label{eq:DP1}
% \end{align}
% \begin{align}
%     V^c_t&(\pi_t) = \min_{\gamma_t \in \mathcal{B}_t} \mathbb{E}[k_t(X_t, U_t) + \\ \notag 
%         &V^c_{t+1}(\delta_{X^0_t}(x^0),\hat{\eta}^1_t(x^0_t,u_t),\hat{\eta}^2_t(x^0_t,u_t)) | \Pi_t = \pi_t, \Gamma_t = \gamma_t]\label{eq:DP1}
% \end{align}
% \red{write the new dynamic DP in terms of general DP}
%  The coordinator's optimal strategy is to pick the minimizing prescription  for each time and each $\pi^a_t$ in problem P1a and $\pi^c_t$ in problem P1c.
% \end{corollary}


The optimal cost in each problem is the expectation of value function at time $t=1$ evaluated at prior belief and initial global state $X^0_1$. Since value functions are same for both the problems P1a and P1c, optimal costs $J^{*a}$ and $J^{*c}$ are equal.
Therefore using Lemma 1 and the above argument,
\begin{equation}
    J^{*a} = J^{*b} = J^{*c}.
\end{equation}

% Let $\mathcal{B}$ be the space of functions from $\mathcal{X}$ to $\Delta(\mathcal{U})$. For a $\gamma \in \mathcal{B}$ and $x \in \mathcal{X}$, $\gamma(x)$ is a probability distribution on $\mathcal{U}$. Let $\gamma(x;u)$ denote the probability assigned to $u \in \mathcal{U}$ under the probability distribution $\gamma(x)$.
% \begin{theorem}\label{thm:dpP1a}
% The value functions in Problem P1a for the coordinator's dynamic program are as follows: Define $V_{T+1}(\pi_{T+1}) =0$ for every $\pi_{T+1}$. For $t \leq T$ and  for any realization $\pi^1_t,\pi^2_t$ of $\Pi^1_t,\Pi^2_t$ respectively, define
% \red{belief update are the same}
% \begin{align}
%     &V^a_{t}(\pi^1_t,\pi^2_t,x^0_t) :=\min_{\gamma_t \in \mathcal{B}}\sum_{x}\sum_{u}\pi^1_t(x^{1})\pi^2_t(x^{2})\gamma_t(x^{1};u^1)\gamma_t(x^{2};u^2)\notag\\
%     &\times\delta_{x^0_t}(x^0)[c_t(x,u)+V_{t+1}(\eta^{1a}_t( \pi^1_{t},\gamma_t,u_t),\eta^{2a}_t( \pi^2_{t},\gamma_t,u_t))]
%  \end{align}
% \end{theorem}

% \begin{theorem}\label{thm:dpP1c}
% The value functions in Problem P1c for the coordinator's dynamic program are as follows: Define $V_{T+1}(\pi_{T+1}) =0$ for every $\pi_{T+1}$. For $t \leq T$ and  for any realization $\pi^1_t,\pi^2_t$ of $\Pi^1_t,\Pi^2_t$ respectively, define

% \begin{align}
%     &V^c_{t}(\pi^1_t,\pi^2_t) :=\min_{\gamma_t \in \mathcal{B}}\sum_{x}\sum_{u}\pi^1_t(x^{1})\pi^2_t(x^{2})\gamma_t(x^{1};u^1)\gamma_t(x^{2};u^2)\notag\\
%     &\times\delta_{X^0_t}(x^0)[c_t(x,u)+V_{t+1}(\eta^{1c}_t( \pi^1_{t},\gamma_t,u_t),\eta^{2c}_t( \pi^2_{t},\gamma_t,u_t))]
%  \end{align}
% \end{theorem}
%The optimal strategy for problem P1a is also optimal for problem P1c as the coordinator's dynamic program are equivalent in both the problems.
